Toward Immersive Communications in 6G

The sixth generation (6G) networks are expected to enable immersive communications and bridge the physical and the virtual worlds. Integrating extended reality, holography, and haptics, immersive communications will revolutionize how people work, entertain, and communicate by enabling lifelike interactions. However, the unprecedented demand for data transmission rate and the stringent requirements on latency and reliability create challenges for 6G networks to support immersive communications. In this survey article, we present the prospect of immersive communications and investigate emerging solutions to the corresponding challenges for 6G. First, we introduce use cases of immersive communications, in the fields of entertainment, education, and healthcare. Second, we present the concepts of immersive communications, including extended reality, haptic communication, and holographic communication, their basic implementation procedures, and their requirements on networks in terms of transmission rate, latency, and reliability. Third, we summarize the potential solutions to addressing the challenges from the aspects of communication, computing, and networking. Finally, we discuss future research directions and conclude this study.

==> Horizons in Computer Science (4)/solution_frontiers.tex <==
\subsection{Common Networking Solutions}

\subsubsection{Content Prediction}



\textbf{Hologram compression}: For current real-time video conferencing systems, media codecs are able to provide compression ratios from 250:1 up to 1000:1 in local devices or MEC servers to reduce the required data rate \citep{selinis2020internet, Ericsson2022}.
Similar to data compression solutions in 2D video transmission, format conversion and data compression should also be applied to reduce the data rate required for holographic communication by minimizing overall data size of the content to be transmitted.
For the LFV, the authors in \citep{mekuria2016design} proposed a lossy real-time color-encoding method exploiting interframe redundancy in point clouds, where a 2D array compression was used for LFV sequence considering the similarity between two image frames. 
Moreover, considering the strong correlation among different views in the hologram, multi-view coding (MVC) for LFV-based streaming was proposed in \citep{xiang2016big}, by analyzing both the horizontal and vertical correlations between 2 adjacent tiles, to reach a higher compression rate resulting in a lower data size.

\subsubsection{Advanced Physical Layer Techniques}

\textbf{TeraHertz}: In order to transmit high-resolution holograms, holographic communication needs up to data rate of Tbps, while current 5G networks can not support such a large bandwidth requirement \citep{shahraki2021comprehensive, david20186g}.
TeraHertz (THz), with spectrum frequencies between the mmWave and optical bands, is expected to be an important physical layer innovation in 6G \citep{jornet2011channel}. 
Featuring higher frequency and larger bandwidth compared with mmWave in 5G, THz can better support immersive communications, as well as allow the flexible network deployments by replacing wired link to THz links \citep{elayan2019terahertz, chen2019survey, tataria20216g}.
In addition, to overcome the severe propagation loss of THz communication, dense deployment and extremely narrowbeam forming can effectively improve communication reliability \citep{8766143}.
However, due to the absorption and reflection properties in the THz regime, the deployment of the THz-based devices and infrastructures still needs to be investigated to optimize communication efficiency \citep{aazhang2019key}.

\subsubsection{Multi-Tier Computing}

\textbf{Multi-tier computing in holographic communication}: In holographic communication, the data from different sensors need to be fused to form a 3D representation of the target object \citep{Javidi05}, which is rendered and reconstructed at the receiver side after data transmission. 
However, the computation capability of local devices is limited and may lead to a large processing delay considering the end-to-end delay requirement due to the high workload of the data fusion and rendering \citep{hu2017survey}. 
Cloud computing is therefore introduced to support high computation workloads for data processing in holographic communication. 
Specifically, transmitting massive data and computing tasks to the cloud may result in a high delay \citep{wang2022task}, which cannot adequately support real-time holographic communication. 
To achieve a low-latency and high computational capacity for data processing in 6G networks, a multi-tier computing scheme can be utilized for holographic communications, which combines the computation resources in the cloud server, MEC servers, and local devices \citep{yang2018meets, wang2022task}.
By integrating computing resources in different layer of networks, content can be processed among multiple servers.
For instance, split rendering was introduced where the MEC server and local device can cooperatively decode and render contents in the holographic communication \citep{Ericsson2022}, which can provide a flexible computing resource management to satisfy the bandwidth and delay requirement through multi-tier computing.

==> solution_frontiers.tex <==
\subsection{Common Networking Solutions}

\subsubsection{Content Prediction}



\textbf{Hologram compression}: For current real-time video conferencing systems, media codecs are able to provide compression ratios from 250:1 up to 1000:1 in local devices or MEC servers to reduce the required data rate \citep{selinis2020internet, Ericsson2022}.
Similar to data compression solutions in 2D video transmission, format conversion and data compression should also be applied to reduce the data rate required for holographic communication by minimizing overall data size of the content to be transmitted.
For the LFV, the authors in \citep{mekuria2016design} proposed a lossy real-time color-encoding method exploiting interframe redundancy in point clouds, where a 2D array compression was used for LFV sequence considering the similarity between two image frames. 
Moreover, considering the strong correlation among different views in the hologram, multi-view coding (MVC) for LFV-based streaming was proposed in \citep{xiang2016big}, by analyzing both the horizontal and vertical correlations between 2 adjacent tiles, to reach a higher compression rate resulting in a lower data size.

\subsubsection{Advanced Physical Layer Techniques}

\textbf{TeraHertz}: In order to transmit high-resolution holograms, holographic communication needs up to data rate of Tbps, while current 5G networks can not support such a large bandwidth requirement \citep{shahraki2021comprehensive, david20186g}.
TeraHertz (THz), with spectrum frequencies between the mmWave and optical bands, is expected to be an important physical layer innovation in 6G \citep{jornet2011channel}. 
Featuring higher frequency and larger bandwidth compared with mmWave in 5G, THz can better support immersive communications, as well as allow the flexible network deployments by replacing wired link to THz links \citep{elayan2019terahertz, chen2019survey, tataria20216g}.
In addition, to overcome the severe propagation loss of THz communication, dense deployment and extremely narrowbeam forming can effectively improve communication reliability \citep{8766143}.
However, due to the absorption and reflection properties in the THz regime, the deployment of the THz-based devices and infrastructures still needs to be investigated to optimize communication efficiency \citep{aazhang2019key}.

\subsubsection{Multi-Tier Computing}

\textbf{Multi-tier computing in holographic communication}: In holographic communication, the data from different sensors need to be fused to form a 3D representation of the target object \citep{Javidi05}, which is rendered and reconstructed at the receiver side after data transmission. 
However, the computation capability of local devices is limited and may lead to a large processing delay considering the end-to-end delay requirement due to the high workload of the data fusion and rendering \citep{hu2017survey}. 
Cloud computing is therefore introduced to support high computation workloads for data processing in holographic communication. 
Specifically, transmitting massive data and computing tasks to the cloud may result in a high delay \citep{wang2022task}, which cannot adequately support real-time holographic communication. 
To achieve a low-latency and high computational capacity for data processing in 6G networks, a multi-tier computing scheme can be utilized for holographic communications, which combines the computation resources in the cloud server, MEC servers, and local devices \citep{yang2018meets, wang2022task}.
By integrating computing resources in different layer of networks, content can be processed among multiple servers.
For instance, split rendering was introduced where the MEC server and local device can cooperatively decode and render contents in the holographic communication \citep{Ericsson2022}, which can provide a flexible computing resource management to satisfy the bandwidth and delay requirement through multi-tier computing.
